Building a real-time physical layer labeled data logging facility for 6G research

This work describes the architecture and vision of designing and implementing a new test infrastructure for 6G physical layer research at KU Leuven. The Testbed is designed for physical layer research and experimentation following several emerging trends, such as cell-free networking, integrated communication, sensing, open disaggregated Radio Access Networks, AI-Native design, and multiband operation. The software is almost entirely based on free and open-source software, making contributing and reusing any component easy. The open Testbed is designed to provide real-time and labeled data on all parts of the physical layer, from raw IQ data to synchronization statistics, channel state information, or symbol/bit/packet error rates. Real-time labeled datasets can be collected by synchronizing the physical layer data logging with a positioning and motion capture system. One of the main goals of the design is to make it open and accessible to external users remotely. Most tests and data captures can easily be automated, and experiment code can be remotely deployed using standard containers (e.g., Docker or Podman). Finally, the paper describes how the Testbed can be used for our research on joint communication and sensing, over-the-air synchronization, distributed processing, and AI in the loop.

==> processingpipeline.tex <==

\begin{figure}
\begin{tikzpicture}[
    % This will show the frame around the figure
    show background rectangle]

   % Place first 6 items
    \node[module] (I1) {0-RAN};
    \node[module, below=of I1] (I2) {Near-RT RIC};
    \node[module, below=of I2] (I3) {O-DU};
    \node[module=1cm, left= 3mm of I1] (I1left) {Labeling};
        \node[module=1cm, left= 3mm of I2] (I2left) {CSI labeling};
    \node[module=1cm, left= 3mm of I3] (I3left) {CSI estimation};
    \node[module=1cm, below=8mm of I3] (I5) {Item-5};
    \node[module=1cm, left= 3mm of I5] (I4) {FGPA X410};
    \node[module=1cm, right= 3mm of I5] (I6) {Item-6};
    \node[module=1cm, below=8mm of I5] (I8) {Item-8};
     \node[module=1cm, left= 3mm of I8] (I7) {Radio X410};
    \node[module=1cm, right= 3mm of I8] (I9) {Item-9};
    % Inner box around Items 3-6
    \node[fit=(I4) (I6) (I7), draw, inner sep=2mm] (fit3) {};
    \node[fit=(I2left) (I3left) (I2), draw, inner sep=2mm] (fit2) {};

    % Outer box around all left items
    %\node[fit=(fit3) (I1), draw, inner sep=2mm] (fit1) {};
    % Connections
    %\foreach \i in {4,5,6}
    %    \draw[->] (I3)--(I\i);
    %\draw[->] (I2)--(I1);
    \draw[->] (I2)--(I3);
    \draw[->] (I2left)--(I3left);
    \draw[->] (fit2)--(fit3);
    \draw[->] (I4)--(I7);
    \draw[->] (I5)--(I8);
    \draw[->] (I6)--(I9);


    

    % Items 7-8-9. Item 7 as label of Item-8
   % \node[module, right=2cm of {I2-|fit1.east}, 
        label={[yshift=5mm, font=\sffamily]Item-7}] 
        (I8) {Item-8};
    %\node[module, below=of I8] (I9) {Item-9};
    %outer box around items 8-9
    %\node[fit={(I9) (I9|-fit1.south) (I9|-fit1.north)}, draw, inner xsep=5mm, inner ysep=-\pgflinewidth] (fit8) {};

    %arrow between boxes
    %\draw[<->,dashed] (fit1)--(fit8);

    %upper label
    %\path (fit1.north east)--node[above=3mm, font=\sffamily\bfseries] (arc) {Architecture} (fit8.north west);

\end{tikzpicture}

\end{figure}

